Rewarding Novel Deductions: Solver-guided Process Supervision for Logical Reasoning

Logical reasoning remains a major challenge for large language models (LLMs), particularly on structured problems that require precise constraint tracking, consistency preservation, and multi-step deduction. This challenge is especially acute for small-scale LLMs, which are more prone to producing inconsistent, redundant, or brittle reasoning trajectories. Existing approaches for improving logical reasoning largely optimize for final-answer correctness, providing only weak supervision over the intermediate reasoning process. In this work, we propose SPRING: (Solver-guided Process Rewards for Novel LogIcal ReasoNing Step Generation). SPRING uses an SMT solver as a training-time verifier of intermediate reasoning steps to provide process-level supervision. It introduces the notion of a novel reasoning step, namely, a step that is logically valid, consistent with the evolving reasoning state, and not already implied by previously accepted non-contradictory deductions. Based on this solver-based assessment, it designs process rewards that encourage novel inferential progress while penalizing contradictory and uninformative reasoning steps. Evaluation across three logical reasoning benchmarks: ZebraLogic, AR-LSAT, and Knights and Knaves, and four LLMs shows that SPRING consistently outperforms base LLMs, outcome-only reward baselines, and Logic-LM. On ZebraLogic, SPRING improves puzzle accuracy by up to 49.71 and 15.43 points over the base LLM and strongest outcome-only baseline, respectively. On AR-LSAT, it improves overall accuracy by up to 64.43 and 11.39 percentage points over the base LLM and strongest outcome-only baseline, respectively. On Knights and Knaves, SPRING achieves up to 93.14 puzzle accuracy and 96.05 person accuracy.

==> Tab_Fig_tex/tab1_Res.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison across different LLMs on the ZebraLogic benchmark.}
\label{tab:results_zebralogic}
\small
\resizebox{0.50\columnwidth}{!}{%
\begin{tabular}{llcc}
\toprule
\textbf{LLM} & \textbf{System} & \textbf{Puzzle Acc.} $\uparrow$ & \textbf{Cell Acc.} $\uparrow$ \\
\midrule

\multirow{5}{*}{Qwen3-1.7B}
& Base-LLM-NL   & 11.14 & 35.04 \\
& OR-NL         & 38.57 & 49.87 \\
\cmidrule(lr){2-4}
& Base-LLM-INT  & 31.85 & 41.45 \\
& OR-INT        & 36.00 & 46.09 \\
\cmidrule(lr){2-4}
& \OurMODEL{} (--Novelty) & 19.28 & 59.62 \\
& \OurMODEL{}             & \textbf{54.00} & \textbf{59.87} \\
\midrule

\multirow{5}{*}{Qwen3-4B-Thinking}
& Base-LLM-NL   & 24.00 & 24.00 \\
& OR-NL         & 67.28 & 68.30 \\
\cmidrule(lr){2-4}
& Base-LLM-INT  & 17.00 & 23.32 \\
& OR-INT        & 66.14 & 72.72 \\
\cmidrule(lr){2-4}
& \OurMODEL{} (--Novelty) & 61.42 & 68.27 \\
& \OurMODEL{}             & \textbf{73.71} & \textbf{81.52} \\
\bottomrule
\end{tabular}}
\vspace{-3.7ex}
\end{table}

==> Tab_Fig_tex/tab2_Res.tex <==
\begin{table*}[b!]
\centering
\caption{Performance comparison across different LLMs on AR-LSAT by problem type.}
\label{tab:ar_lsat_results}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{LLM} & \textbf{System} & \textbf{Ordering} $\uparrow$ & \textbf{Grouping} $\uparrow$ & \textbf{Assignment} $\uparrow$ & \textbf{Overall} $\uparrow$ \\
\midrule

\multirow{6}{*}{Qwen3-1.7B}
& Base-LLM-NL               & 16.07 & 24.48 & 0.00  & 13.52 \\
& OR-NL                     & 19.64 & 40.81 & 1.44  & 20.63 \\
\cmidrule(lr){2-6}
& Base-LLM-INT              & 23.21 & 24.48 & 14.49 & 20.73 \\
& OR-INT                    & 35.71 & 51.02 & 24.63 & 37.12 \\
\cmidrule(lr){2-6}
& \OurMODEL{} (--Novelty)   & 34.82 & 55.10 & 46.37 & 45.43 \\
& \textbf{\OurMODEL{}}      & \textbf{41.07} & \textbf{57.14} & \textbf{49.56} & \textbf{49.26} \\
\midrule

\multirow{6}{*}{Qwen3-4B-Thinking}
& Base-LLM-NL               & 6.25  & 18.36 & 0.00  & 8.20 \\
& OR-NL                     & 25.00 & 65.30 & 10.14 & 33.48 \\
\cmidrule(lr){2-6}
& Base-LLM-INT              & 6.26  & 14.28 & 5.50  & 8.68 \\
& OR-INT                    & 61.60 & 79.59 & 65.21 & 68.80 \\
\cmidrule(lr){2-6}
& \OurMODEL{} (--Novelty)   & 63.39 & 77.55 & 66.66 & 69.20 \\
& \textbf{\OurMODEL{}}      & \textbf{69.64} & \textbf{81.63} & \textbf{69.56} & \textbf{73.61} \\

\bottomrule
\end{tabular}}
\end{table*}

==> Tab_Fig_tex/tab3_res_combined_bkup.tex <==
\begin{table*}[t]
\centering
\caption{\OurMODEL{} performance comparison across different LLMs on ZebraLogic and AR-LSAT.}
\label{tab:combined_results}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.83\textwidth}{!}{%
\begin{tabular}{llcc|cccc}
\toprule
\multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{System}} 
& \multicolumn{2}{c|}{\textbf{ZebraLogic}} 
& \multicolumn{4}{c}{\textbf{AR-LSAT (Acc.)}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-8}
& 
& \textbf{Puzzle Acc.} $\uparrow$ 
& \textbf{Cell Acc.} $\uparrow$
& \textbf{Ordering} $\uparrow$
& \textbf{Grouping} $\uparrow$
& \textbf{Assignment} $\uparrow$
& \textbf{Overall} $\uparrow$ \\
\midrule

\multirow{6}{*}{Qwen3-1.7B}
& Base-NL             & 11.14 & 35.04 & 16.07 & 24.48 & 0.00  & 13.52 \\
& OR-NL                   & 38.57 & 49.87 & 19.64 & 40.81 & 1.44  & 20.63 \\
\cmidrule(lr){2-8}
& Base-INT            & 31.85 & 41.45 & 23.21 & 24.48 & 14.49 & 20.73 \\
& OR-INT                  & 36.00 & 46.09 & 35.71 & 51.02 & 24.63 & 37.12 \\
\cmidrule(lr){2-8}
& \OurMODEL{} (--N) & 19.28 & 59.62 & 34.82 & 55.10 & 46.37 & 45.43 \\
& \textbf{\OurMODEL{}}    & \textbf{54.00} & \textbf{59.87} & \textbf{41.07} & \textbf{57.14} & \textbf{49.56} & \textbf{49.26} \\
\midrule

\multirow{6}{*}{Qwen3-4B-Thinking}
& Base-NL             & 24.00 & 24.00 & 6.25  & 18.36 & 0.00  & 8.20 \\
& OR-NL                   & 67.28 & 68.30 & 25.00 & 65.30 & 10.14 & 33.48 \\
\cmidrule(lr){2-8}
& Base-INT            & 17.00 & 23.32 & 6.26  & 14.28 & 5.50  & 8.68 \\
& OR-INT                  & 66.14 & 72.72 & 61.60 & 79.59 & 65.21 & 68.80 \\
\cmidrule(lr){2-8}
& \OurMODEL{} (--N) & 61.42 & 68.27 & 63.39 & 77.55 & 66.66 & 69.20 \\
& \textbf{\OurMODEL{}}    & \textbf{73.71} & \textbf{81.52} & \textbf{69.64} & \textbf{81.63} & \textbf{69.56} & \textbf{73.61} \\
\bottomrule



\multirow{6}{*}{Phi4-Reasoning}
& Base-NL              & x.x & x.x & 12.5  & 24.48 & 17.39  & x.x \\
& OR-NL                & x.x & x.x & x.x  & x.x & x.x  & x.x \\
\cmidrule(lr){2-8}
& Base-INT             & 18.71 & 20.27 & 0.0  & 18.36 & 2.89  & x.x \\
& OR-INT               & 49.00 & 53.54 & 23.21  & 46.93 & 26.08  & x.x \\
\cmidrule(lr){2-8}
& \OurMODEL{} (--N)    & 53.71 & 56.34 & 22.32 & 42.85 & 24.63 & x.x \\
& \textbf{\OurMODEL{}} & 55.71 & 59.52 & 26.78 & 51.02 & 34.78 & x.x \\

\bottomrule


\multirow{6}{*}{Qwen3-8B}
& Base-NL              & x.x & x.x & x.x  & x.x & x.x  & x.x \\
& OR-NL                & x.x & x.x & x.x  & x.x & x.x  & x.x \\
\cmidrule(lr){2-8}
& Base-INT             & x.x & x.x & x.x  & x.x & x.x  & x.x \\
& OR-INT               & x.x & x.x & x.x  & x.x & x.x  & x.x \\
\cmidrule(lr){2-8}
& \OurMODEL{} (--N)    & x.x & x.x & x.x & x.x & x.x & x.x \\
& \textbf{\OurMODEL{}} & x.x & x.x & x.x & x.x & x.x & x.x \\
\bottomrule

\end{tabular}}
\vspace{-3.7ex}
\end{table*}

==> Tab_Fig_tex/tab5_analyses_detailed_v1.tex <==
\begin{table*}[t]
\centering
\caption{Validation metrics by inferred puzzle size for \texttt{jobid\_276924\_epoch\_28\_valid\_feedback.jsonl}. Size is extracted from \texttt{pid} as \(A\times B\).}
\label{tab:sizewise_metrics}
\small
\setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c}
\toprule
\textbf{Size} & \textbf{\#Samples} & \textbf{Cell Acc.} & \textbf{SAT-Rate} & \textbf{\#Novel-Steps} & \textbf{Puzzle Acc.} \\
\midrule
2x2 & 23 & 1.000 & 0.957 & 0.96 & 1.000 \\
2x3 & 27 & 1.000 & 1.000 & 2.15 & 1.000 \\
2x4 & 31 & 0.935 & 0.871 & 2.84 & 0.935 \\
2x5 & 26 & 0.904 & 0.923 & 2.96 & 0.846 \\
2x6 & 29 & 0.877 & 0.828 & 2.83 & 0.793 \\
3x2 & 33 & 0.970 & 0.939 & 3.24 & 0.970 \\
3x3 & 29 & 0.980 & 1.000 & 3.97 & 0.931 \\
3x4 & 26 & 0.964 & 1.000 & 5.69 & 0.923 \\
3x5 & 29 & 0.931 & 0.931 & 6.62 & 0.931 \\
3x6 & 28 & 0.905 & 0.929 & 3.43 & 0.857 \\
4x2 & 26 & 0.859 & 0.885 & 3.12 & 0.846 \\
4x3 & 30 & 0.883 & 0.900 & 4.13 & 0.867 \\
4x4 & 27 & 0.896 & 0.815 & 4.85 & 0.852 \\
4x5 & 29 & 0.864 & 0.828 & 3.86 & 0.759 \\
4x6 & 26 & 0.801 & 0.923 & 5.08 & 0.692 \\
5x2 & 29 & 0.931 & 0.931 & 3.28 & 0.931 \\
5x3 & 29 & 0.984 & 0.931 & 4.14 & 0.966 \\
5x4 & 31 & 0.836 & 0.871 & 5.94 & 0.677 \\
5x5 & 28 & 0.540 & 0.714 & 2.54 & 0.393 \\
5x6 & 30 & 0.421 & 0.667 & 2.27 & 0.200 \\
6x2 & 27 & 0.947 & 0.852 & 4.70 & 0.852 \\
6x3 & 23 & 0.931 & 0.870 & 5.70 & 0.826 \\
6x4 & 24 & 0.669 & 0.708 & 3.12 & 0.458 \\
6x5 & 27 & 0.201 & 0.704 & 1.11 & 0.000 \\
6x6 & 33 & 0.253 & 0.455 & 1.58 & 0.030 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Tab_Fig_tex/tab_ablation1.tex <==
\begin{table}[h]
\centering
\caption{Ablation-Analyses using Interleaved Prompt and Qwen3-4B-Thinking.}
\label{tab:ablation}
\resizebox{\textwidth}{!}{
\begin{tabular}{l l c c c c c c}
\toprule
\textbf{LLM} & \textbf{System} & Puzzle Acc. & Cell Acc. & \#Parsed-Steps (Avg.) & \#Valid (\%)  & \#Novel (\%) & \#Contradictions (\%) \\
\midrule


\multirow{4}{*}{Qwen3-4B-Thinking}
& --N           & 61.42 & 68.27 & 47.68    & 29.73   & 9.10   & 1.56 \\
& --C           & -.-   & -.-   & -.-      & -.-   & -.-   & -.- \\
& -- NC         & 66.14 & 72.72 & 25.72    & 31.84 & 10.27 & 0.75 \\
& \OurMODEL{}   & 73.71 & 81.52 & 35.81    & 46.61 & 16.91 & 0.55 \\

\bottomrule
\end{tabular}}
\end{table}



\eat{

--N: 
BASE_n_steps_total	35.1992
BASE_n_steps_parsed_ok	16.1875
BASE_n_steps_valid	15.9922
BASE_n_steps_novel_inc_clues	8.0820
BASE_n_non_valid_contradiction	0.1602

--C:

--NC:


SPRING: 
BASE_n_steps_total	22.3682
BASE_n_steps_parsed_ok	11.0000
BASE_n_steps_valid	10.9535
BASE_n_steps_novel_inc_clues	4.4709
BASE_n_non_valid_contradiction	0.0465


}

==> Tab_Fig_tex/tab_ablation2.tex <==
\begin{table*}[t]
\centering
\caption{Normalized reasoning-trace quality across three reward settings. All quantities are computed over correctly solved cases only.}
\label{tab:three_way_trace_quality}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\textbf{Setting} & \textbf{Parsed / Total} & \textbf{Valid / Parsed} & \textbf{Valid / Total} & \textbf{Novel / Valid} & \textbf{Contradictions / Total} \\
\midrule
Novelty \(=0.4\)                    & 0.492 & 0.996 & 0.490 & 0.408 & 0.0021 \\
Novelty \(=0.0\)                    & 0.460 & 0.988 & 0.454 & 0.505 & 0.0045 \\
Novelty \(=0.0\), Contradiction \(=0.0\) & 0.347 & 0.953 & 0.330 & 0.365 & 0.0120 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> Tab_Fig_tex/tab_ablation3.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of three reward settings. \#Correct and Puzzle Acc. are computed over the full validation log. All remaining columns are averages over correctly solved cases only, i.e., instances with \(\texttt{Puzzle Acc.}=1.0\).}
\label{tab:three_way_trace_comparison}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c}
\toprule
\textbf{Setting} & \textbf{\#Total} & \textbf{\#Correct} & \textbf{Puzzle Acc.} & \textbf{SAT-rate} & \textbf{\#Total-steps} & \textbf{\#Parsed-steps} & \textbf{\#Valid-steps} & \textbf{\#Novel-steps} & \textbf{\#Contradictions} \\
\midrule
Novelty \(=0.4\)                    & 700 & 516 & 0.737 & 0.965 & 22.37 & 11.00 & 10.95 & 4.47 & 0.047 \\
Novelty \(=0.0\)                    & 476 & 256 & 0.538 & 0.941 & 35.20 & 16.19 & 15.99 & 8.08 & 0.160 \\
Novelty \(=0.0\), Contradiction \(=0.0\) & 700 & 463 & 0.661 & 0.814 & 34.82 & 12.07 & 11.51 & 4.20 & 0.417 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> Tab_Fig_tex/tab_ablation4.tex <==
\begin{table*}[t]
\centering
\caption{Quality of reasoning traces on correctly solved cases. All trace statistics are averaged only over instances with \(\texttt{Puzzle Acc.}=1.0\). Higher is better for Puzzle Acc., SAT-rate, Parsed/Total, and Valid/Parsed. Lower is better for Steps/Solved and Contradictions/100 Steps.}
\label{tab:trace_quality_correct}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c}
\toprule
\textbf{Setting} & \textbf{\#Correct / \#Total} & \textbf{Puzzle Acc.} & \textbf{SAT-rate} & \textbf{Steps / Solved} & \textbf{Parsed / Total} & \textbf{Valid / Parsed} & \textbf{Contradictions / 100 Steps} \\
\midrule
Novelty \(=0.4\) & \textbf{516 / 700} & \textbf{0.737} & \textbf{0.965} & \textbf{22.37} & \textbf{0.492} & \textbf{0.996} & \textbf{0.21} \\
Novelty \(=0.0\) & 256 / 476 & 0.538 & 0.941 & 35.20 & 0.460 & 0.988 & 0.45 \\
Novelty \(=0.0\), Contradiction \(=0.0\) & 463 / 700 & 0.661 & 0.814 & 34.82 & 0.347 & 0.953 & 1.20 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> Tab_Fig_tex/tab_ablation5.tex <==
\begin{table*}[t]
\centering
\caption{Behavior of reasoning traces on incorrect cases only, i.e., instances with \(\texttt{Puzzle Acc.}=0\). Lower is better for Failed Steps and Contradictions. Higher Cell Acc. indicates that even failed traces may preserve some partial local structure.}
\label{tab:trace_quality_incorrect}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{0.92\textwidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\textbf{Setting} & \textbf{\#Incorrect} & \textbf{Failed Steps} & \textbf{Parsed / Total} & \textbf{Valid / Parsed} & \textbf{Contradictions / 100 Steps} \\
\midrule
Novelty \(=0.4\) & \textbf{184} & \textbf{9.39} & \textbf{0.495} & \textbf{0.991} & \textbf{0.46} \\
Novelty \(=0.0\) & 220 & 49.10 & 0.384 & 0.824 & 6.77 \\
Novelty \(=0.0\), Contradiction \(=0.0\) & 237 & 11.23 & 0.305 & 0.912 & 2.52 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> Tab_Fig_tex/tab_ablation6.tex <==
\begin{table}[t]
\centering
\caption{Novel-step quality on correctly solved cases. Raw novel-step counts are shown together with normalized efficiency and reliability measures. Higher is better for Novel/Total and Valid/Novel; lower is better for Contradictions/Novel.}
\label{tab:novel_step_quality}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
\textbf{Setting} & \textbf{\#Novel-steps} & \textbf{Novel / Total} & \textbf{Valid / Novel} & \textbf{Contradictions / Novel} \\
\midrule
Novelty \(=0.4\) & 4.47 & 0.200 & 2.45 & \textbf{0.010} \\
Novelty \(=0.0\) & 8.08 & 0.230 & 1.98 & 0.020 \\
Novelty \(=0.0\), Contradiction \(=0.0\) & 4.20 & 0.121 & \textbf{2.74} & 0.099 \\
\bottomrule
\end{tabular}%
}
\end{table}
